Swift: Rethinking RDMA Control Plane for Elastic Computing

Elastic computing enables dynamic scaling to meet workload demands, and Remote Direct Memory Access (RDMA) enhances this by providing high-throughput, low-latency network communication. However, integrating RDMA into elastic computing remains a challenge, particularly in control plane operations for RDMA connection setup. This paper revisits the assumptions of prior work on high-performance RDMA for elastic computing, and reveals that extreme microsecond-level control plane optimizations are often unnecessary. By challenging the conventional beliefs on the slowness of user-space RDMA control plane and the difficulty of user-space RDMA resource sharing, we uncover new design opportunities. Our key insight is that user-space RDMA connection setup can be significantly improved with caching, while RDMA resources can be efficiently shared among processes using fork. In light of this, we propose Swift, a simple yet effective solution that co-designs RDMA with a serverless framework to optimize performance for elastic computing. At its very core, Swift handles cold and warm serverless requests by swiftly initializing the RDMA control plane with cache-optimized libibverbs, and manages fork requests by leveraging the RDMA's fork capability. Implemented with OpenWhisk, Swift delivers 30.56-46.50% higher average throughput and 18.55-37.21% lower latency, at a cost of 6.5% control plane overhead, compared to prior solutions.

==> table/libibverbs-api-time.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{lccc}
\toprule
\textbf{\libibverbs APIs} & \textbf{Time~($\mu$s)} & \textbf{User-space} & \textbf{Kernel-space} \\
\midrule
\ibvgetdevicelist & 1888 & 1231 & 657 \\
\ibvopendevice & 22992 & 21235 & 1757 \\
\ibvallocpd & 209 & 89 & 120 \\
\ibvregmr & 112 & 63 & 49 \\
\ibvcreateqp & 866 & 583 & 283 \\
\ibvmodifyqp & 365 & 203 & 162 \\
\bottomrule
\end{tabular}
\caption{Performance of \libibverbs API calls in user-space and kernel-space.}
\label{tab:libibverbs-api-time}
\end{table}

==> table/rdma-overhead.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Scenario} & \textbf{Task Launch Time} & \textbf{RDMA Connection Setup} & \textbf{RDMA Control Plane Overhead} \\
\midrule
Cold Start \& Others & Several hundred ms to several s & 20-30 ms & Low to moderate \\
Warm Start & Tens of ms & 20-30 ms & High \\
Fork Start & Sub-ms to a few ms & 20-30 ms & Very high \\
\bottomrule
\end{tabular}
\caption{Comparison of RDMA connection setup overhead with task launch time.}
\label{tab:rdma-overhead}
\end{table*}
